From Driver to Supervisor: Comparing Cognitive Load and EEG-based Attentional Resource Allocation across Automation Levels

With increasing automation, drivers' roles transition from active operators to passive system supervisors, affecting their behaviour and cognitive processes. This study addresses the attentional resource allocation and subjective cognitive load during manual, SAE Level 2, and SAE Level 3 driving in a realistic environment. An experiment was conducted on a test track with 30 participants using a prototype automated vehicle. While driving, participants were subjected to a passive auditory oddball task and their electroencephalogram was recorded. The study analysed the amplitude of the P3a event-related potential component elicited by novel environmental stimuli, an objective measure of attentional resource allocation. The subjective cognitive load was assessed using the NASA Task Load Index. Results showed no significant difference in subjective cognitive load between manual and Level 2 driving, but a decrease in subjective cognitive load in Level 3 driving. The P3a amplitude was highest during manual driving, indicating increased attentional resource allocation to environmental sounds compared to Level 2 and Level 3 driving. This may suggest that during automated driving, drivers allocate fewer attentional resources to processing environmental information. It remains unclear whether the decreased processing of environmental stimuli in automated driving is due to top-down attention control (leading to attention withdrawal) or bottom-up competition for resources induced by cognitive load. This study provides novel empirical evidence on resource allocation and subjective cognitive load in automated driving. The findings highlight the importance of managing drivers' attention and cognitive load with implications for enhancing automation safety and the design of user interfaces.

==> references.tex <==
@inproceedings{manstetten2021,
author = {Manstetten, Dietrich and Beruscha, Frank and Bieg, Hans-Joachim and Kobiela, Fanny and Korthauer, Andreas and Krautter, Wolfgang and Marberger, Claus},
title = {The Evolution of Driver Monitoring Systems: A Shortened Story on Past, Current and Future Approaches How Cars Acquire Knowledge About the Driver's State},
year = {2021},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
doi = {https://doi.org/10.1145/3406324.3425896},
articleno = {60},
numpages = {6},
location = {Oldenburg, Germany},
series = {MobileHCI '20}
}

@article{gevins2003neurophysiological,
  title={Neurophysiological measures of cognitive workload during human-computer interaction},
  author={Gevins, Alan and Smith, Michael E},
  journal={Theoretical issues in ergonomics science},
  volume={4},
  number={1-2},
  pages={113--131},
  year={2003},
  publisher={Taylor \& Francis}
}

@phdthesis{kraus2020psychological,
  title={Psychological processes in the formation and calibration of trust in automation},
  author={Kraus, Johannes Maria},
  year={2020},
  school={Universit{\"a}t Ulm}
}

@article{pauzie2008method,
  title={A method to assess the driver mental workload: The driving activity load index (DALI)},
  author={Pauzi{\'e}, Annie},
  journal={IET Intelligent Transport Systems},
  volume={2},
  number={4},
  pages={315--322},
  year={2008},
  publisher={IET}
}


@article{fabiani1996naming,
  title={Naming norms for brief environmental sounds: Effects of age and dementia},
  author={Fabiani, Monica and Kazmerski, Victoria A and Cycowicz, Yael M and Friedman, David},
  journal={Psychophysiology},
  volume={33},
  number={4},
  pages={462--475},
  year={1996},
  publisher={Wiley Online Library}
}

@inproceedings{hart2006nasa,
  title={NASA-task load index (NASA-TLX); 20 years later},
  author={Hart, Sandra G},
  booktitle={Proceedings of the human factors and ergonomics society annual meeting},
  volume={50},
  number={9},
  pages={904--908},
  year={2006},
  organization={Sage publications Sage CA: Los Angeles, CA}
}

@article{klug2022zapline,
  title={Zapline-plus: A Zapline extension for automatic and adaptive removal of frequency-specific noise artifacts in M/EEG},
  author={Klug, Marius and Kloosterman, Niels A},
  journal={Human Brain Mapping},
  year={2022},
  publisher={Wiley Online Library}
}

@article{de2020zapline,
  title={ZapLine: A simple and effective method to remove power line artifacts},
  author={de Cheveign{\'e}, Alain},
  journal={NeuroImage},
  volume={207},
  pages={116356},
  year={2020},
  publisher={Elsevier}
}

@article{klug2022bemobil,
  title={The BeMoBIL Pipeline for automated analyses of multimodal mobile brain and body imaging data},
  author={Klug, Marius and Jeung, Sein and Wunderlich, Anna and Gehrke, Lukas and Protzak, Janna and Djebbara, Zakaria and Argubi-Wollesen, Andreas and Wollesen, Bettina and Gramann, Klaus},
  journal={bioRxiv},
  year={2022},
  publisher={Cold Spring Harbor Laboratory}
}

@article{fagnant2015preparing,
  title={Preparing a nation for autonomous vehicles: opportunities, barriers and policy recommendations},
  author={Fagnant, Daniel J and Kockelman, Kara},
  journal={Transportation Research Part A: Policy and Practice},
  volume={77},
  pages={167--181},
  year={2015},
  publisher={Elsevier}
}

@article{sae2016j3016,
  title={J3016-Taxonomy and definitions for terms related to on-road motor vehicle automated driving systems},
  author={SAE, SoAEI},
  journal={Surface Vehicle Recommended Practive},
  year={2016}
}

@article{szHucs2022road,
  title={Road Safety Analysis of Autonomous Vehicles: An Overview},
  author={Sz{\H{u}}cs, Herman and H{\'e}zer, Jozefin},
  journal={Periodica Polytechnica Transportation Engineering},
  volume={50},
  number={4},
  pages={426--434},
  year={2022}
}

@article{yamani2018theoretical,
  title={A theoretical model of human-automation interaction grounded in resource allocation policy during automated driving},
  author={Yamani, Yusuke and Horrey, William J},
  journal={International Journal of Human Factors and Ergonomics},
  volume={5},
  number={3},
  pages={225--239},
  year={2018},
  publisher={Inderscience Publishers (IEL)}
}

@article{schroger1998attentional,
  title={Attentional orienting and reorienting is indicated by human event-related brain potentials},
  author={Schr{\"o}ger, Erich and Wolff, Christian},
  journal={Neuroreport},
  volume={9},
  number={15},
  pages={3355--3358},
  year={1998},
  publisher={LWW}
}

@article{scheer2016steering,
  title={Steering demands diminish the early-P3, late-P3 and RON components of the event-related potential of task-irrelevant environmental sounds},
  author={Scheer, Menja and B{\"u}lthoff, Heinrich H and Chuang, Lewis L},
  journal={Frontiers in human neuroscience},
  volume={10},
  pages={73},
  year={2016},
  publisher={Frontiers Media SA}
}

@incollection{shahid2011karolinska,
  title={Karolinska sleepiness scale (KSS)},
  author={Shahid, Azmeh and Wilkinson, Kate and Marcu, Shai and Shapiro, Colin M},
  booktitle={STOP, THAT and one hundred other sleep scales},
  pages={209--210},
  year={2011},
  publisher={Springer}
}


@article{wilson2020driver,
  title={Driver trust \& mode confusion in an on-road study of level-2 automated vehicle technology},
  author={Wilson, Kyle M and Yang, Shiyan and Roady, Trey and Kuo, Jonny and Lenn{\'e}, Michael G},
  journal={Safety Science},
  volume={130},
  pages={104845},
  year={2020},
  publisher={Elsevier}
}

@article{de2014effects,
  title={Effects of adaptive cruise control and highly automated driving on workload and situation awareness: A review of the empirical evidence},
  author={De Winter, Joost CF and Happee, Riender and Martens, Marieke H and Stanton, Neville A},
  journal={Transportation research part F: traffic psychology and behaviour},
  volume={27},
  pages={196--217},
  year={2014},
  publisher={Elsevier}
}

@article{banks2016keep,
  title={Keep the driver in control: Automating automobiles of the future},
  author={Banks, Victoria A and Stanton, Neville A},
  journal={Applied ergonomics},
  volume={53},
  pages={389--395},
  year={2016},
  publisher={Elsevier}
}

@article{young2007s,
  title={What's skill got to do with it? Vehicle automation and driver mental workload},
  author={Young, Mark S and Stanton, Neville A},
  journal={Ergonomics},
  volume={50},
  number={8},
  pages={1324--1339},
  year={2007},
  publisher={Taylor \& Francis}
}

@inproceedings{stapel2017driver,
  title={Driver behavior and workload in an on-road automated vehicle},
  author={Stapel, Jork and Mullakkal-Babu, Freddy Antony and Happee, Riender},
  booktitle={Proceedings of the RSS2017 Conference},
  year={2017}
}

 @misc{robinson_2023, title={Police in Germany chase tesla for 15 minutes after driver turns on autopilot and 'goes to sleep'}, url={https://news.sky.com/story/police-in-germany-chase-tesla-for-15-minutes-after-driver-turns-on-autopilot-and-goes-to-sleep-12778306}, journal={Sky News}, publisher={Sky}, author={Robinson, James}, year={2023}, month={Jan}} 

  @misc{klippenstein_2023, title={Exclusive: Surveillance footage of Tesla crash on SF's Bay Bridge hours after Elon Musk announces "self-driving" feature}, url={https://theintercept.com/2023/01/10/tesla-crash-footage-autopilot/}, journal={The Intercept}, publisher={The Intercept}, author={Klippenstein, Ken}, year={2023}, month={Jan}} 

  @article{parasuraman1997humans,
  title={Humans and automation: Use, misuse, disuse, abuse},
  author={Parasuraman, Raja and Riley, Victor},
  journal={Human factors},
  volume={39},
  number={2},
  pages={230--253},
  year={1997},
  publisher={SAGE Publications Sage CA: Los Angeles, CA}
}

@inproceedings{merat2009drivers,
  title={How do drivers behave in a highly automated car?},
  author={Merat, Natasha and Jamson, A Hamish},
  booktitle={Driving Assesment Conference},
  volume={5},
  number={2009},
  year={2009},
  organization={University of Iowa}
}

@article{zhou2021effects,
  title={Effects of explanation-based knowledge regarding system functions and driver’s roles on driver takeover during conditionally automated driving: A test track study},
  author={Zhou, Huiping and Kamijo, Keita and Itoh, Makoto and Kitazaki, Satoshi},
  journal={Transportation research part F: traffic psychology and behaviour},
  volume={77},
  pages={1--9},
  year={2021},
  publisher={Elsevier}
}

  @incollection{bainbridge1983ironies,
  title={Ironies of automation},
  author={Bainbridge, Lisanne},
  booktitle={Analysis, design and evaluation of man--machine systems},
  pages={129--135},
  year={1983},
  publisher={Elsevier}
}

@inproceedings{wintersberger2022user,
  title={User Experience Evaluation of SAE Level 3 Driving on a Test Track},
  author={Wintersberger, Philipp and Shadeghian-Borojeni, Shadan and Schartm{\"u}ller, Clemens and Frison, Anna-Katharina and Riener, Andreas},
  booktitle={2022 IEEE Intelligent Vehicles Symposium (IV)},
  pages={1409--1414},
  year={2022},
  organization={IEEE}
}

@inproceedings{frison2019you,
  title={Why do you like to drive automated? a context-dependent analysis of highly automated driving to elaborate requirements for intelligent user interfaces},
  author={Frison, Anna-Katharina and Wintersberger, Philipp and Liu, Tianjia and Riener, Andreas},
  booktitle={Proceedings of the 24th international conference on intelligent user interfaces},
  pages={528--537},
  year={2019}
}

@article{vogelpohl2019asleep,
  title={Asleep at the automated wheel—Sleepiness and fatigue during highly automated driving},
  author={Vogelpohl, Tobias and K{\"u}hn, Matthias and Hummel, Thomas and Vollrath, Mark},
  journal={Accident Analysis \& Prevention},
  volume={126},
  pages={70--84},
  year={2019},
  publisher={Elsevier}
}

@article{bieg2020task,
  title={Task load of professional drivers during level 2 and 3 automated driving},
  author={Bieg, Hans-Joachim and Daniilidou, Constantina and Michel, Britta and Sprung, Anna},
  journal={Proceedings of the Human Factors and Ergonomics Society Europe},
  pages={41--52},
  year={2020}
}

 @inproceedings{kundinger2020driver,
  title={Driver drowsiness in automated and manual driving: insights from a test track study},
  author={Kundinger, Thomas and Riener, Andreas and Sofra, Nikoletta and Weigl, Klemens},
  booktitle={Proceedings of the 25th International Conference on Intelligent User Interfaces},
  pages={369--379},
  year={2020}
}

 @inproceedings{michael2006sustained,
  title={Sustained attention and hypovigilance: The effect of environmental monotony on continuous task performance and implications for road safety},
  author={Michael, Rebecca and Meuter, Renata},
  booktitle={Proceedings of the Australasian road safety research, policing and education conference},
  volume={10},
  year={2006},
  organization={Monash University}
}

@article{madigan2018effect,
  title={The effect of varying levels of vehicle automation on drivers’ lane changing behaviour},
  author={Madigan, Ruth and Louw, Tyron and Merat, Natasha},
  journal={PloS one},
  volume={13},
  number={2},
  pages={e0192190},
  year={2018},
  publisher={Public Library of Science San Francisco, CA USA}
}

@inproceedings{large2017exploring,
  title={Exploring the behaviour of distracted drivers during different levels of automation in driving},
  author={Large, David R and Banks, Victoria A and Burnett, Gary and Baverstock, Sarah and Skrypchuk, Lee},
  booktitle={Proceedings of the 5th international conference on driver distraction and inattention (DDI2017), March},
  pages={20--22},
  year={2017}
}

@article{matthews2019dangerous,
  title={Dangerous intersections? A review of studies of fatigue and distraction in the automated vehicle},
  author={Matthews, Gerald and Neubauer, Catherine and Saxby, Dyani J and Wohleber, Ryan W and Lin, Jinchao},
  journal={Accident Analysis \& Prevention},
  volume={126},
  pages={85--94},
  year={2019},
  publisher={Elsevier}
}

@inproceedings{biondi201880,
  title={80 MPH and out-of-the-loop: Effects of real-world semi-automated driving on driver workload and arousal},
  author={Biondi, Francesco N and Lohani, Monika and Hopman, Rachel and Mills, Sydney and Cooper, Joel M and Strayer, David L},
  booktitle={Proceedings of the human factors and ergonomics society annual meeting},
  volume={62},
  number={1},
  pages={1878--1882},
  year={2018},
  organization={SAGE Publications Sage CA: Los Angeles, CA}
}

@article{stapel2019automated,
  title={Automated driving reduces perceived workload, but monitoring causes higher cognitive load than manual driving},
  author={Stapel, Jork and Mullakkal-Babu, Freddy Antony and Happee, Riender},
  journal={Transportation research part F: traffic psychology and behaviour},
  volume={60},
  pages={590--605},
  year={2019},
  publisher={Elsevier}
}
@article{mcwilliams2021underload,
  title={Underload on the road: measuring vigilance decrements during partially automated driving},
  author={McWilliams, Thomas and Ward, Nathan},
  journal={Frontiers in psychology},
  volume={12},
  pages={631364},
  year={2021},
  publisher={Frontiers Media SA}
}

@article{lohani2021no,
  title={No difference in arousal or cognitive demands between manual and partially automated driving: a multi-method on-road study},
  author={Lohani, Monika and Cooper, Joel M and Erickson, Gus G and Simmons, Trent G and McDonnell, Amy S and Carriero, Amanda E and Crabtree, Kaedyn W and Strayer, David L},
  journal={Frontiers in neuroscience},
  pages={627},
  year={2021},
  publisher={Frontiers}
}

@inproceedings{sibi2017assessing,
  title={Assessing driver cortical activity under varying levels of automation with functional near infrared spectroscopy},
  author={Sibi, Srinath and Baiters, Stephanie and Mok, Brian and Steiner, Martin and Ju, Wendy},
  booktitle={2017 IEEE Intelligent Vehicles Symposium (IV)},
  pages={1509--1516},
  year={2017},
  organization={IEEE}
}

@article{varhelyi2021driving,
  title={Driving with and without automation on the motorway--an observational study},
  author={V{\'a}rhelyi, Andr{\'a}s and Kaufmann, Clemens and Johnsson, Carl and Almqvist, Sverker},
  journal={Journal of Intelligent Transportation Systems},
  volume={25},
  number={6},
  pages={587--608},
  year={2021},
  publisher={Taylor \& Francis}
}

@inproceedings{lohani2020driver,
  title={Driver Arousal and Workload Under Partial Vehicle Automation: A Pilot Study},
  author={Lohani, Monika and Cooper, Joel M and Erickson, Gus G and Simmons, Trent G and McDonnell, Amy S and Carriero, Amanda E and Crabtree, Kaedyn W and Strayer, David L},
  booktitle={Proceedings of the Human Factors and Ergonomics Society Annual Meeting},
  volume={64},
  number={1},
  pages={1955--1959},
  year={2020},
  organization={SAGE Publications Sage CA: Los Angeles, CA}
}

@article{kim2023partially,
  title={Partially automated driving has higher workload than manual driving: An on-road comparison of three contemporary vehicles with SAE Level 2 features},
  author={Kim, Jisun and Revell, Kirsten and Langdon, Pat and Bradley, Mike and Politis, Ioannis and Thompson, Simon and Skrypchuk, Lee and O'Donoghue, Jim and Richardson, Joy and Stanton, Neville A},
  journal={Human Factors and Ergonomics in Manufacturing \& Service Industries},
  volume={33},
  number={1},
  pages={40--54},
  year={2023},
  publisher={Wiley Online Library}
}

@article{mcdonnell2021your,
  title={This is your brain on Autopilot: Neural indices of driver workload and engagement during partial vehicle automation},
  author={McDonnell, Amy S and Simmons, Trent G and Erickson, Gus G and Lohani, Monika and Cooper, Joel M and Strayer, David L},
  journal={Human factors},
  pages={00187208211039091},
  year={2021},
  publisher={SAGE Publications Sage CA: Los Angeles, CA}
}

 @inproceedings{kundinger2020driver,
  title={Driver drowsiness in automated and manual driving: insights from a test track study},
  author={Kundinger, Thomas and Riener, Andreas and Sofra, Nikoletta and Weigl, Klemens},
  booktitle={Proceedings of the 25th International Conference on Intelligent User Interfaces},
  pages={369--379},
  year={2020}
}

@article{eriksson2017transition,
  title={Transition to manual: Comparing simulator with on-road control transitions},
  author={Eriksson, Alexander and Banks, VA and Stanton, NA},
  journal={Accident Analysis \& Prevention},
  volume={102},
  pages={227--234},
  year={2017},
  publisher={Elsevier}
}

@article{groh2019simulation,
  title={Simulation and its contribution to evaluate highly automated driving functions},
  author={Groh, Korbinian and Wagner, Sebastian and Kuehbeck, Thomas and Knoll, Alois},
  journal={SAE International Journal of Advances and Current Practices in Mobility},
  volume={1},
  number={2019-01-0140},
  pages={539--549},
  year={2019}
}

@book{kahneman1973attention,
  title={Attention and effort},
  author={Kahneman, Daniel},
  volume={1063},
  year={1973},
  publisher={Citeseer}
}

@inproceedings{longo2016mental,
  title={Mental workload in medicine: foundations, applications, open problems, challenges and future perspectives},
  author={Longo, Luca},
  booktitle={2016 ieee 29th international symposium on computer-based medical systems (cbms)},
  pages={106--111},
  year={2016},
  organization={IEEE}
}

@article{wickens2002multiple,
  title={Multiple resources and performance prediction},
  author={Wickens, Christopher D},
  journal={Theoretical issues in ergonomics science},
  volume={3},
  number={2},
  pages={159--177},
  year={2002},
  publisher={Taylor \& Francis}
}

@article{wickens2008multiple,
  title={Multiple resources and mental workload},
  author={Wickens, Christopher D},
  journal={Human factors},
  volume={50},
  number={3},
  pages={449--455},
  year={2008},
  publisher={SAGE Publications Sage CA: Los Angeles, CA}
}

@article{wickens1980structure,
  title={The structure of attentional resources},
  author={Wickens, Christopher D},
  journal={Attention and performance VIII},
  volume={8},
  pages={239--257},
  year={1980}
}

@article{de1996measurement,
  title={The measurement of drivers' mental workload},
  author={De Waard, Dick and Brookhuis, KA},
  year={1996},
  publisher={Groningen University, Traffic Research Center Netherlands}
}

@article{meister1976behavioral,
  title={Behavioral foundations of system development.},
  author={Meister, David},
  year={1976},
  publisher={John Wiley \& Sons}
}

@article{yerkes1908relation,
  title={The relation of strength of stimulus to rapidity of habit-formation},
  author={Yerkes, Robert Mearns and Dodson, John D and others},
  year={1908},
  publisher={Editorial Office, Denison University}
}

@article{warm2008vigilance,
  title={Vigilance requires hard mental work and is stressful},
  author={Warm, Joel S and Parasuraman, Raja and Matthews, Gerald},
  journal={Human factors},
  volume={50},
  number={3},
  pages={433--441},
  year={2008},
  publisher={SAGE Publications Sage CA: Los Angeles, CA}
}

@article{de1991assessing,
  title={Assessing driver status: a demonstration experiment on the road},
  author={De Waard, Dick and Brookhuis, Karel A},
  journal={Accident analysis \& prevention},
  volume={23},
  number={4},
  pages={297--307},
  year={1991},
  publisher={Elsevier}
}

@incollection{eggemeier2020workload,
  title={Workload assessment in multi-task environments},
  author={Eggemeier, F Thomas and Wilson, Glenn F and Kramer, Arthur F and Damos, Diane L},
  booktitle={Multiple-task performance},
  pages={207--216},
  year={2020},
  publisher={CRC Press}
}

@article{de2014self,
  title={Self-report scales alone cannot capture mental workload},
  author={de Waard, Dick and Lewis-Evans, Ben},
  journal={Cognition, technology \& work},
  volume={16},
  number={3},
  pages={303--305},
  year={2014},
  publisher={Springer}
}

@article{grant2013measuring,
  title={Measuring surgeons’ mental workload with a time-based secondary task},
  author={Grant, Russell C and Carswell, C Melody and Lio, Cindy H and Seales, W Brent},
  journal={Ergonomics in Design},
  volume={21},
  number={1},
  pages={7--11},
  year={2013},
  publisher={SAGE Publications Sage CA: Los Angeles, CA}
}

@article{lohani2019review,
  title={A review of psychophysiological measures to assess cognitive states in real-world driving},
  author={Lohani, Monika and Payne, Brennan R and Strayer, David L},
  journal={Frontiers in human neuroscience},
  volume={13},
  pages={57},
  year={2019},
  publisher={Frontiers Media SA}
}
@article{kramer1995assessment,
  title={Assessment of mental workload with task-irrelevant auditory probes},
  author={Kramer, Arthur F and Trejo, Leonard J and Humphrey, Darryl},
  journal={Biological psychology},
  volume={40},
  number={1-2},
  pages={83--100},
  year={1995},
  publisher={Elsevier}
}

@article{papanicolaou1984probe,
  title={Probe evoked potentials: theory, method and applications},
  author={Papanicolaou, Andrew C and Johnstone, Jack},
  journal={International Journal of Neuroscience},
  volume={24},
  number={2},
  pages={107--131},
  year={1984},
  publisher={Taylor \& Francis}
}

@article{sirevaag1993assessment,
  title={Assessment of pilot performance and mental workload in rotary wing aircraft},
  author={Sirevaag, Erik J and Kramer, Arthur F and REISWEBER, CHRISTOPHER D WICKENS MARK and STRAYER, DAVID L and GRENELL, JAMES F},
  journal={Ergonomics},
  volume={36},
  number={9},
  pages={1121--1140},
  year={1993},
  publisher={Taylor \& Francis}
}

 @book{luck_2014, place={Cambridge, MA}, title={An introduction to the event-related potential technique}, publisher={The MIT Press}, author={Luck, Steven J.}, year={2014}} 

@article{escera1998neural,
  title={Neural mechanisms of involuntary attention to acoustic novelty and change},
  author={Escera, Carles and Alho, Kimmo and Winkler, Istv{\'a}n and N{\"a}{\"a}t{\"a}nen, Risto},
  journal={Journal of cognitive neuroscience},
  volume={10},
  number={5},
  pages={590--604},
  year={1998},
  publisher={MIT Press One Rogers Street, Cambridge, MA 02142-1209, USA journals-info~…}
}

@article{escera2007role,
  title={Role of mismatch negativity and novelty-P3 in involuntary auditory attention.},
  author={Escera, Carles and Corral, MJ},
  journal={Journal of psychophysiology},
  volume={21},
  number={3-4},
  pages={251},
  year={2007},
  publisher={Hogrefe \& Huber Publishers}
}

@article{escera2003attention,
  title={Attention capture by auditory significant stimuli: semantic analysis follows attention switching},
  author={Escera, Carles and Yago, Elena and Corral, Maria-Jos{\'e} and Corbera, Silvia and Nu{\~n}ez, M Isabel},
  journal={European Journal of Neuroscience},
  volume={18},
  number={8},
  pages={2408--2412},
  year={2003},
  publisher={Wiley Online Library}
}


@article{byers1989traditional,
  title={Traditional and raw task load index (TLX) correlations: Are paired comparisons necessary},
  author={Byers, James C and Bittner, AC and Hill, Susan G},
  journal={Advances in industrial ergonomics and safety},
  volume={1},
  pages={481--485},
  year={1989},
  publisher={Taylor \& Francis London}
}

@article{pion2019iclabel,
  title={ICLabel: An automated electroencephalographic independent component classifier, dataset, and website},
  author={Pion-Tonachini, Luca and Kreutz-Delgado, Ken and Makeig, Scott},
  journal={NeuroImage},
  volume={198},
  pages={181--197},
  year={2019},
  publisher={Elsevier}
}


@article{kok1997event,
  title={Event-related-potential (ERP) reflections of mental resources: a review and synthesis},
  author={Kok, A},
  journal={Biological psychology},
  volume={45},
  number={1-3},
  pages={19--56},
  year={1997},
  publisher={Elsevier}
}

@article{kothe2012lab,
  title={Lab Streaming Layer (LSL)-A software framework for synchronizing a large array of data collection and stimulation devices},
  author={Kothe, C and Medine, D and Boulay, C and Grivich, M and Stenner, T},
  journal={Available online: https://github.com/sccn/labstreaminglayer (accessed on March 10 2023)},
  year={2019}
}

@article{kothe2012xdfimport,
  title={XDFimport Plugin},
  author={Kothe, C},
  journal={Swartz Center for Computational Neuroscience UCSD, Available online: https://github.com/xdf-modules/xdf-EEGLAB (accessed on March 10 2023)},
  year={2012}
}


@article{delorme2011eeglab,
  title={EEGLAB, SIFT, NFT, BCILAB, and ERICA: new tools for advanced EEG processing},
  author={Delorme, Arnaud and Mullen, Tim and Kothe, Christian and Acar, Zeynep Akalin and Bigdely-Shamlo, Nima and Vankov, Andrey and Makeig, Scott},
  journal={Computational intelligence and neuroscience},
  volume={2011},
  pages={10--10},
  year={2011},
  publisher={Hindawi Limited London, UK, United Kingdom}
}


@article{delorme2004eeglab,
  title={EEGLAB: an open source toolbox for analysis of single-trial EEG dynamics including independent component analysis},
  author={Delorme, Arnaud and Makeig, Scott},
  journal={Journal of neuroscience methods},
  volume={134},
  number={1},
  pages={9--21},
  year={2004},
  publisher={Elsevier}
}

@article{kok2001utility,
  title={On the utility of P3 amplitude as a measure of processing capacity},
  author={Kok, Albert},
  journal={Psychophysiology},
  volume={38},
  number={3},
  pages={557--577},
  year={2001},
  publisher={Cambridge University Press}
}

@article{polich2007updating,
  title={Updating P300: an integrative theory of P3a and P3b},
  author={Polich, John},
  journal={Clinical neurophysiology},
  volume={118},
  number={10},
  pages={2128--2148},
  year={2007},
  publisher={Elsevier}
}

 @article{hari_pelizzone_mäkelä_hällström_leinonen_lounasmaa_1987, title={Neuromagnetic responses of the human auditory cortex to on- and offsets of noise bursts: Réponses neuromagnétiques du cortex auditif humain à l'établissement et l'extinction de salves de bruit}, volume={26}, DOI={10.3109/00206098709078405}, number={1}, journal={International Journal of Audiology}, author={Hari, R. and Pelizzone, M. and Mäkelä, J. P. and Hällström, J. and Leinonen, L. and Lounasmaa, O. V.}, year={1987}, pages={31–43}} 

 @article{muller2007evidence,
  title={Evidence for the auditory P3a reflecting an automatic process: elicitation during highly-focused continuous visual attention},
  author={Muller-Gass, Alexandra and Macdonald, Margaret and Schr{\"o}ger, Erich and Sculthorpe, Lauren and Campbell, Kenneth},
  journal={Brain research},
  volume={1170},
  pages={71--78},
  year={2007},
  publisher={Elsevier}
}

@article{ghani2020erp,
  title={ERP based measures of cognitive workload: A review},
  author={Ghani, Usman and Signal, Nada and Niazi, Imran Khan and Taylor, Denise},
  journal={Neuroscience \& Biobehavioral Reviews},
  volume={118},
  pages={18--26},
  year={2020},
  publisher={Elsevier}
}

@article{van2021effect,
  title={The effect of cognitive load on auditory susceptibility during automated driving},
  author={Van der Heiden, Remo MA and Kenemans, J Leon and Donker, Stella F and Janssen, Christian P},
  journal={Human factors},
  pages={0018720821998850},
  year={2021},
  publisher={SAGE Publications Sage CA: Los Angeles, CA}
}

@misc{githubGitHubSccnlabstreaminglayer,
	author = {Chadwick Boulay},
	title = {{G}it{H}ub - sccn/labstreaminglayer: {L}ab{S}treaming{L}ayer super repository comprising submodules for {L}{S}{L} and associated apps. --- github.com},
	howpublished = {\url{https://github.com/sccn/labstreaminglayer}},
	year = {2023},
	note = {[Accessed 19-Jan-2023]},
}

@article{blair1993alternative,
  title={An alternative method for significance testing of waveform difference potentials},
  author={Blair, R Clifford and Karniski, Walt},
  journal={Psychophysiology},
  volume={30},
  number={5},
  pages={518--524},
  year={1993},
  publisher={Wiley Online Library}
}

@article{hemmelmann2004multivariate,
  title={Multivariate tests for the evaluation of high-dimensional EEG data},
  author={Hemmelmann, Claudia and Horn, Manfred and Reiterer, Susanne and Schack, B{\"a}rbel and S{\"u}sse, Thomas and Weiss, Sabine},
  journal={Journal of Neuroscience Methods},
  volume={139},
  number={1},
  pages={111--120},
  year={2004},
  publisher={Elsevier}
}

@book{manly2018randomization,
  title={Randomization, Bootstrap and Monte Carlo Methods in Biology: Texts in Statistical Science},
  author={Manly, Bryan FJ},
  year={2018},
  publisher={chapman and hall/CRC}
}

@article{friedman2001novelty,
  title={The novelty P3: an event-related brain potential (ERP) sign of the brain's evaluation of novelty},
  author={Friedman, David and Cycowicz, Yael M and Gaeta, Helen},
  journal={Neuroscience \& Biobehavioral Reviews},
  volume={25},
  number={4},
  pages={355--373},
  year={2001},
  publisher={Elsevier}
}

@article{luck2017get,
  title={How to get statistically significant effects in any ERP experiment (and why you shouldn't)},
  author={Luck, Steven J and Gaspelin, Nicholas},
  journal={Psychophysiology},
  volume={54},
  number={1},
  pages={146--157},
  year={2017},
  publisher={Wiley Online Library}
}

@article{cahn2013event,
  title={Event-related delta, theta, alpha and gamma correlates to auditory oddball processing during Vipassana meditation},
  author={Cahn, B Rael and Delorme, Arnaud and Polich, John},
  journal={Social cognitive and affective neuroscience},
  volume={8},
  number={1},
  pages={100--111},
  year={2013},
  publisher={Oxford University Press}
}

@article{kramer2020physiological,
  title={Physiological metrics of mental workload: A review of recent progress},
  author={Kramer, Arthur F},
  journal={Multiple-task performance},
  pages={279--328},
  year={2020},
  publisher={CRC Press}
}

@article{charles2019measuring,
  title={Measuring mental workload using physiological measures: A systematic review},
  author={Charles, Rebecca L and Nixon, Jim},
  journal={Applied ergonomics},
  volume={74},
  pages={221--232},
  year={2019},
  publisher={Elsevier}
}

@article{wester2010effects,
  title={Effects of alcohol on attention orienting and dual-task performance during simulated driving: An event-related potential study},
  author={Wester, Anne E and Verster, Joris C and Volkerts, Edmund R and B{\"o}cker, Koen BE and Kenemans, J Leon},
  journal={Journal of psychopharmacology},
  volume={24},
  number={9},
  pages={1333--1348},
  year={2010},
  publisher={Sage Publications Sage UK: London, England}
}

@article{wester2008event,
  title={Event-related potentials and secondary task performance during simulated driving},
  author={Wester, Anne E and B{\"o}cker, Koen BE and Volkerts, Edmund R and Verster, Joris C and Kenemans, J Leon},
  journal={Accident Analysis \& Prevention},
  volume={40},
  number={1},
  pages={1--7},
  year={2008},
  publisher={Elsevier}
}

@article{van2018susceptibility,
  title={Susceptibility to audio signals during autonomous driving},
  author={Van der Heiden, Remo MA and Janssen, Christian P and Donker, Stella F and Hardeman, Lotte ES and Mans, Keri and Kenemans, J Leon},
  journal={PloS one},
  volume={13},
  number={8},
  pages={e0201963},
  year={2018},
  publisher={Public Library of Science San Francisco, CA USA}
}

@article{kavnovsky2003impact,
  title={The impact of motor activity on intracerebral ERPs: P3 latency variability in modified auditory odd-ball paradigms involving a motor task},
  author={Ka{\v{n}}ovsk{\`y}, Petr and Streitov{\'a}, Hana and Klajblov{\'a}, Hana and Bare{\v{s}}, Martin and Daniel, Pavel and Rektor, Ivan},
  journal={Neurophysiologie Clinique/Clinical Neurophysiology},
  volume={33},
  number={4},
  pages={159--168},
  year={2003},
  publisher={Elsevier}
}

@article{kubler2009brain,
  title={A brain--computer interface controlled auditory event-related potential (P300) spelling system for locked-in patients},
  author={K{\"u}bler, Andrea and Furdea, Adrian and Halder, Sebastian and Hammer, Eva Maria and Nijboer, Femke and Kotchoubey, Boris},
  journal={Annals of the New York Academy of Sciences},
  volume={1157},
  number={1},
  pages={90--100},
  year={2009},
  publisher={Wiley Online Library}
}

@article{solis2019event,
  title={Event-related potentials as indices of mental workload while using an in-vehicle information system},
  author={Sol{\'\i}s-Marcos, Ignacio and Kircher, Katja},
  journal={Cognition, Technology \& Work},
  volume={21},
  pages={55--67},
  year={2019},
  publisher={Springer}
}

@book{spence2020crossmodal,
  title={Crossmodal Attention Applied: Lessons for Driving},
  author={Spence, Charles and Soto-Faraco, Salvador},
  year={2020},
  publisher={Cambridge University Press}
}

@article{just2008decrease,
  title={A decrease in brain activation associated with driving when listening to someone speak},
  author={Just, Marcel Adam and Keller, Timothy A and Cynkar, Jacquelyn},
  journal={Brain research},
  volume={1205},
  pages={70--80},
  year={2008},
  publisher={Elsevier}
}
@article{palmiero2019neural,
  title={Neural correlates of simulated driving while performing a secondary task: a review},
  author={Palmiero, Massimiliano and Piccardi, Laura and Boccia, Maddalena and Baralla, Francesca and Cordellieri, Pierluigi and Sgalla, Roberto and Guidoni, Umberto and Giannini, Anna Maria},
  journal={Frontiers in Psychology},
  volume={10},
  pages={1045},
  year={2019},
  publisher={Frontiers Media SA}
}


@article{ciaramitaro2017cross,
  title={Cross-modal attention influences auditory contrast sensitivity: Decreasing visual load improves auditory thresholds for amplitude-and frequency-modulated sounds},
  author={Ciaramitaro, Vivian M and Chow, Hiu Mei and Eglington, Luke G},
  journal={Journal of Vision},
  volume={17},
  number={3},
  pages={20--20},
  year={2017},
  publisher={The Association for Research in Vision and Ophthalmology}
}

@article{wahn2015vision,
  title={Vision and haptics share spatial attentional resources and visuotactile integration is not affected by high attentional load},
  author={Wahn, Basil and K{\"o}nig, Peter},
  journal={Multisensory Research},
  volume={28},
  number={3-4},
  pages={371--392},
  year={2015},
  publisher={Brill}
}

@article{chen2017hemispheric,
  title={Hemispheric asymmetry: Looking for a novel signature of the modulation of spatial attention in multisensory processing},
  author={Chen, Yi-Chuan and Spence, Charles},
  journal={Psychonomic bulletin \& review},
  volume={24},
  pages={690--707},
  year={2017},
  publisher={Springer}
}

@article{ho2007multisensory,
  title={Multisensory in-car warning signals for collision avoidance},
  author={Ho, Cristy and Reed, Nick and Spence, Charles},
  journal={Human factors},
  volume={49},
  number={6},
  pages={1107--1114},
  year={2007},
  publisher={SAGE Publications Sage CA: Los Angeles, CA}
}

@article{lunn2019multisensory,
  title={Multisensory enhancement of attention depends on whether you are already paying attention},
  author={Lunn, J and Sjoblom, A and Ward, J and Soto-Faraco, S and Forster, S},
  journal={Cognition},
  volume={187},
  pages={38--49},
  year={2019},
  publisher={Elsevier}
}

@article{gemonet2021car,
  title={Car drivers coping with hazardous events in real versus simulated situations: Declarative, behavioral and physiological data used to assess drivers’ feeling of presence},
  author={Gemonet, Elise and Bougard, Cl{\'e}ment and Masfrand, St{\'e}phane and Honnet, Vincent and Mestre, Daniel R},
  journal={PLoS one},
  volume={16},
  number={2},
  pages={e0247373},
  year={2021},
  publisher={Public Library of Science San Francisco, CA USA}
}

@inproceedings{helton2022national,
  title={The National Aviation and Space Agency Task Load Index (NASA-TLX): Does it Need Updating?},
  author={Helton, William S and Jackson, Kenneth M and N{\"a}swall, Katharina and Humphrey, Bonnie},
  booktitle={Proceedings of the Human Factors and Ergonomics Society Annual Meeting},
  volume={66},
  number={1},
  pages={1245--1249},
  year={2022},
  organization={SAGE Publications Sage CA: Los Angeles, CA}
}

@inproceedings{mckendrick2018deeper,
  title={A deeper look at the NASA TLX and where it falls short},
  author={McKendrick, Ryan D and Cherry, Erin},
  booktitle={Proceedings of the Human Factors and Ergonomics Society Annual Meeting},
  volume={62},
  number={1},
  pages={44--48},
  year={2018},
  organization={SAGE Publications Sage CA: Los Angeles, CA}
}

@inproceedings{hock2018design,
  title={How to design valid simulator studies for investigating user experience in automated driving: review and hands-on considerations},
  author={Hock, Philipp and Kraus, Johannes and Babel, Franziska and Walch, Marcel and Rukzio, Enrico and Baumann, Martin},
  booktitle={Proceedings of the 10th International Conference on Automotive User Interfaces and Interactive Vehicular Applications},
  pages={105--117},
  year={2018}
}

@article{galera2012mind,
  title={Mind wandering and driving: responsibility case-control study},
  author={Gal{\'e}ra, C{\'e}dric and Orriols, Ludivine and M’Bailara, Katia and Laborey, Magali and Contrand, Benjamin and Rib{\'e}reau-Gayon, R{\'e}gis and Masson, Fran{\c{c}}oise and Bakiri, Sarah and Gabaude, Catherine and Fort, Alexandra and others},
  journal={Bmj},
  volume={345},
  year={2012},
  publisher={British Medical Journal Publishing Group}
}

@article{baldwin2017detecting,
  title={Detecting and quantifying mind wandering during simulated driving},
  author={Baldwin, Carryl L and Roberts, Daniel M and Barragan, Daniela and Lee, John D and Lerner, Neil and Higgins, James S},
  journal={Frontiers in human neuroscience},
  volume={11},
  pages={406},
  year={2017},
  publisher={Frontiers Media SA}
}

@article{merat2014transition,
  title={Transition to manual: Driver behaviour when resuming control from a highly automated vehicle},
  author={Merat, Natasha and Jamson, A Hamish and Lai, Frank CH and Daly, Michael and Carsten, Oliver MJ},
  journal={Transportation research part F: traffic psychology and behaviour},
  volume={27},
  pages={274--282},
  year={2014},
  publisher={Elsevier}
}

@article{chun2011taxonomy,
  title={A taxonomy of external and internal attention},
  author={Chun, Marvin M and Golomb, Julie D and Turk-Browne, Nicholas B},
  journal={Annual review of psychology},
  volume={62},
  pages={73--101},
  year={2011},
  publisher={Annual Reviews}
}

@article{wynne2019systematic,
  title={Systematic review of driving simulator validation studies},
  author={Wynne, Rachael A and Beanland, Vanessa and Salmon, Paul M},
  journal={Safety science},
  volume={117},
  pages={138--151},
  year={2019},
  publisher={Elsevier}
}



@article{ryerson2020safety,
  title={Safety at the edge: a safety framework to identify edge conditions in the future transportation system with highly automated vehicles},
  author={Ryerson, Megan S and Long, Carrie S and Scudder, Kristen and Winston, Flaura K},
  journal={Injury prevention},
  volume={26},
  number={4},
  pages={386--390},
  year={2020},
  publisher={BMJ Publishing Group Ltd}
}

@article{baluch2011mechanisms,
  title={Mechanisms of top-down attention},
  author={Baluch, Farhan and Itti, Laurent},
  journal={Trends in neurosciences},
  volume={34},
  number={4},
  pages={210--224},
  year={2011},
  publisher={Elsevier}
}

@article{wang2020salience,
  title={Salience determines attentional orienting in visual selection.},
  author={Wang, Benchi and Theeuwes, Jan},
  journal={Journal of Experimental Psychology: Human Perception and Performance},
  volume={46},
  number={10},
  pages={1051},
  year={2020},
  publisher={American Psychological Association}
}

@article{mole2019getting,
  title={Getting back into the loop: the perceptual-motor determinants of successful transitions out of automated driving},
  author={Mole, Callum D and Lappi, Otto and Giles, Oscar and Markkula, Gustav and Mars, Franck and Wilkie, Richard M},
  journal={Human factors},
  volume={61},
  number={7},
  pages={1037--1065},
  year={2019},
  publisher={Sage Publications Sage CA: Los Angeles, CA}
}

@article{scheer2018auditory,
  title={Auditory task irrelevance: a basis for inattentional deafness},
  author={Scheer, Menja and B{\"u}lthoff, Heinrich H and Chuang, Lewis L},
  journal={Human factors},
  volume={60},
  number={3},
  pages={428--440},
  year={2018},
  publisher={Sage Publications Sage CA: Los Angeles, CA}
}

@inproceedings{brandenburg2014switching,
  title={Switching from manual to automated driving and reverse: Are drivers behaving more risky after highly automated driving?},
  author={Brandenburg, Stefan and Skottke, E-M},
  booktitle={17th international IEEE conference on intelligent transportation systems (ITSC)},
  pages={2978--2983},
  year={2014},
  organization={IEEE}, 
  publisher = {Institute of Electrical and Electronics Engineers (IEEE)}
}


@inproceedings{figalova2023fatigue,
  title={Fatigue and mental underload further pronounced in L3 conditionally automated driving: Results from an EEG experiment on a test track},
  author={Figalov{\'a}, Nikol and Bieg, Hans-Joachim and Schulz, Michael and Pichen, J{\"u}rgen and Baumann, Martin and Chuang, Lewis L and Pollatos, Olga},
  booktitle={Companion Proceedings of the 28th International Conference on Intelligent User Interfaces},
  pages={64--67},
  year={2023}
}

@inproceedings{merat2009bdrivers,
  title={Is Drivers' Situation Awareness Influenced by a Fully Automated Driving Scenario?},
  author={Merat, Natasha and Jamson, A Hamish},
  booktitle={Human factors, security and safety},
  year={2009},
  organization={Shaker Publishing}
}

@article{jamson2013behavioural,
  title={Behavioural changes in drivers experiencing highly-automated vehicle control in varying traffic conditions},
  author={Jamson, A Hamish and Merat, Natasha and Carsten, Oliver MJ and Lai, Frank CH},
  journal={Transportation research part C: emerging technologies},
  volume={30},
  pages={116--125},
  year={2013},
  publisher={Elsevier}
}

@article{stanton2009human,
  title={Human error taxonomies applied to driving: A generic driver error taxonomy and its implications for intelligent transport systems},
  author={Stanton, Neville A and Salmon, Paul M},
  journal={Safety Science},
  volume={47},
  number={2},
  pages={227--237},
  year={2009},
  publisher={Elsevier}
}

@article{bucsuhazy2020human,
  title={Human factors contributing to the road traffic accident occurrence},
  author={Bucsuhazy, Kate{\v{r}}ina and Matuchov{\'a}, Eva and Zuvala, Robert and Moravcov{\'a}, Pavl{\'\i}na and Kost{\'\i}kov{\'a}, Martina and Mikulec, Roman},
  journal={Transportation research procedia},
  volume={45},
  pages={555--561},
  year={2020},
  publisher={Elsevier}
}

@article{bagiella2000mixed,
  title={Mixed-effects models in psychophysiology},
  author={Bagiella, Emilia and Sloan, Richard P and Heitjan, Daniel F},
  journal={Psychophysiology},
  volume={37},
  number={1},
  pages={13--20},
  year={2000},
  publisher={Cambridge University Press}
}

